Breaking Out of the Ivory Tower: A Large-scale Analysis of Patent Citations to HCI Research

What is the impact of human-computer interaction research on industry? While it is impossible to track all research impact pathways, the growing literature on translational research impact measurement offers patent citations as one measure of how industry recognizes and draws on research in its inventions. In this paper, we perform a large-scale measurement study primarily of 70,000 patent citations to premier HCI research venues, tracing how HCI research are cited in United States patents over the last 30 years. We observe that 20.1% of papers from these venues, including 60--80% of papers at UIST and 13% of papers in a broader dataset of SIGCHI-sponsored venues overall, are cited by patents -- far greater than premier venues in science overall (9.7%) and NLP (11%). However, the time lag between a patent and its paper citations is long (10.5 years) and getting longer, suggesting that HCI research and practice may not be efficiently connected.

==> old_findings1.tex <==
\section{Findings}
In this section, we present our main findings on how USPTO patents recognize papers in CHI, CSCW, UIST, and UbiComp (IMWUT). 

\msb{To help me trust these results, it would be helpful as a descriptive outcome to show highly cited patents that cite HCI Research. In other words, is there a way to find example patents that are clearly examples of industry versions of academic research? Can we show actual lineage? Otherwise, the whole time I read this I worry that it's just like a paper that's citing related work because it's roughly relevant but not actually influential.}

%\hancheng{@yuting, add some transition sentences at each subsection, e.g. we further explored XX}
%\yt{done.}
\subsection{RQ1: how many HCI papers are recognized by patents}
We first study the quantity of HCI papers that are later recognized by patents and present a table of top papers cited by patents.
%investigated who are the top patent assignees that cite HCI papers and what are the mostly cited papers by patents, and compared the content of paper vs. Patent over time.   

%\paragraph{\textbf{number of HCI papers over time}}
%\hancheng{merge this paragraph to the next paragraph}

%As shown in Figure ~\ref{fig:f1}, HCI research has grown rapidly over the past $38$ years for all four venues, especially at CHI: from $0$ papers in $1980$ to ~$1500$ in $2018$. This growth is particularly pronounced within the last 10 years. 


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{main_figs/fig_1.png}
    \caption{Left: the number of papers published by each conference per year (red) and the number of papers published in that year that were later cited by at least one patent (green) \msb{change colors for people who are red-green colorblind. I suggest red and blue.}, at ACM CHI, CSCW, UbiComp, and UIST. A substantial proportion of HCI papers are recognized by patents, e.g. $60\%$ - $80\%$ UIST papers are recognized by patents $1990$ - $2010$. \msb{The graphs need language cleaned up. The conference titles are small compared to the legend. paper number should be ``Published'' and cited paper number should be ``Published and later cited by patents''. x axis should be year and y axis should be number of papers. Capitalize all axis titles. cited ratio should be ``percent of published papers later cited by patents'' and the y axis should be a percent and not a number. CSCW did not meet annually until 2008 so there should not be any papers published on those off years. add some whitespace between the facets of the graphs---rows are squished too close together} }
    
    \label{fig:f1}
\end{figure}


%\hancheng{needs to add an aggregated percentage, 18.5\% for all papers} \yt{done. }
\paragraph{\textbf{Proportion of papers that get cited by patents}}
To assess the extent of HCI research being recognized in patents, we first calculated the aggregated proportion of the number of HCI papers at our four venues that were cited by patents. We found $18.5\%$ of HCI papers are recognized by patents in our data. 

\msb{Can you help the reader benchmark if this is a little or a lot? How does this compare to patent citation rates in other CS subfields? Or in non-CS subfields? Is 18\% a lot or a little?}

Investigating temporal patterns, we plot the total number of HCI research papers in each venue published over years, shown in red in Figure~\ref{fig:f1}. HCI research has grown rapidly over the past $38$ years for all four venues, especially at CHI: from $0$ papers in $1980$ to ~$1500$ in $2018$. This growth is particularly pronounced within the last $10$ years. We then counted the total number of HCI papers were cited by patents by the publication year of the paper (green line in Figure~\ref{fig:f1}) and calculated the ratio between the number of HCI papers cited and the total number of HCI paper accepted at a particular year by each venue (blue line in Figure~\ref{fig:f1}) \msb{the zeroes in these graphs are likely data errors or years the conference did not meet? For example, it looks like 0 papers in CHI 1984, and thus ratio 0? Please double check, and if they're not actual zeros, remove them from the graphs so they're not distracting}. The citation ratios start climbing expecially starting around 1990 and persist since then (Figure~\ref{fig:f1}),\footnote{Note that CSCW were held twice a year in the early conference history, which is the reason we observed 0 paper numbers for earlier years every two years till 2010 \msb{remove the zeros from the graph, just graph straight from that meeting to the next meeting, e.g., connect 1990 to 1992 rather than dipping to zero in 1991}} with several conferences observing a third to a half of their papers cited by patents. At UIST in particular, the patent citation ratio reaches $60\%$ - $80\%$ in $1990$ - $2010$.

However, we also observed a decreasing trend in cited ratio after 2015. One possible explanation is that the HCI field is growing much larger, and as a result, the ratio is decreasing. Another possible explanation is the time lag between patent and paper is long, e.g., it might take a decade for a paper to start gathering patent citations, and papers since 2015 are still too young by this metric: this time lag will be further discussed in Section~\ref{sec:patent_recognize}. Thus the data are right censored, i.e., more recent papers have not been fully recognized by patents captured in our dataset.

%This trend can be further corroborated by the number of patents that cite HCI papers over time. 
\paragraph{\textbf{Increasing citations to HCI research in patents.}}
A considerable number of patents cite HCI research. \msb{I have no basis to conclude whether these raw numbers are ``considerable'' or not. What is a lot of patents? What number would be big? Can you help benchmark? Same critique as earlier --- can you help benchmark what is a lot, and what is a little, via references to other CS subfields or other fields?} This raw volume began increasing after $2000$ (Figure~\ref{fig:f2}, and more than quintupled since then at CHI (from around 175 patents per year in 2000 to over 1000 per year in 2014). However, the number of patents plateaus and even decreases a bit in more recent years, e.g. patents that cite CSCW research start to go down around 2014. This could be a result of changes in the demand side, e.g., industry being less interested in novel social computing applications, or on the supply side, e.g., HCI publishing more papers that are not intended to be as industry-relevant. More evidence is needed to derive the mechanisms behind this result, beyond the scope of our current work.

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{main_figs/fig_8.png}
    \caption{Over 1000 CHI papers are cited by a patent each year. The number of patents citing HCI research began rising after 2000 and more than quintupled since then. \msb{Title should be Patents Citing HCI Research}}
    \label{fig:f2}
\end{figure}

\paragraph{\textbf{Top cited papers by patents in HCI}}
%Top cited papers by patents (title, total patent citation, year published) of HCI is shown in Table~\ref{tab:top_HCI}. 

We further examined the HCI papers that were cited the most by patents by each venue (Table~\ref{tab:top_HCI}). Papers highly cited by patents are also highly cited by research. The papers most highly cited by patents are primarily systems work, e.g., building a new system or proposing a new design. This result parallels the earlier observation that UIST has the highest rate of papers cited by patents, since UIST is particularly targeted at new interfaces, software, and technologies. Across the four venues that we selected, CHI and UIST papers have been cited most by patents, followed by CSCW and then UbiComp \msb{this result has nothing to do with ``Top cited papers by patents in HCI''. Also not sure how it's measured --- raw count, or ratio?}. Most papers in this list are published prior 2005; however, the majority of the patents that cite HCI papers come after 2005, indicating again the potential long time lag between paper publication and patent reference in \autoref{sec:patent_recognize}.

\begin{table*}[tb]
\centering
\resizebox{\textwidth}{!}{%    
\begin{tabular}{l l l l}
\toprule
\textbf{Title} & \textbf{Patent citations} & \textbf{Paper citations} & \textbf{Year published} \\
\midrule
\multicolumn{4}{c}{\textbf{CHI}} \\
\midrule
    A multi-touch three dimensional touch-sensitive tablet & 708 & 231& 1985 \\
    PaperLink: a technique for hyperlinking from real paper to electronic content & 200 & 134&1997 \\
    Bringing order to the Web: automatically categorizing search results & 196 & 486 &2000 \\
    A study in two-handed input & 175 & 544&1986 \\
    Generalized fisheye views & 175 & 2180&1986 \\
    SmartSkin: an infrastructure for freehand manipulation on interactive surfaces & 166 & 770&2002 \\
    AppLens and launchTile: two designs for one-handed thumb use on small devices & 159 & 133&2005 \\
    Active click: tactile feedback for touch panels & 156 & 195&2001 \\
    Finding others online: reputation systems for social online spaces & 153 & 100&2002 \\
    Applying electric field sensing to human-computer interfaces & 142 &272 &1995 \\
\midrule
\multicolumn{4}{c}{\textbf{CSCW}} \\
\midrule
    GroupLens: an open architecture for collaborative filtering of netnews & 185 & 5771&1994 \\
    WebSplitter: a unified XML framework for multi-device collaborative Web browsing & 166 &186 &2000 \\
    Blogging as a social activity, or, would you let 900 million people read your diary? & 121 & 584&2004 \\
    MMConf: an infrastructure for building shared multimedia applications & 106 &313 &1990 \\
    An experiment in integrated multimedia conferencing & 103 & 157&1986 \\
    Collaboration using multiple PDAs connected to a PC & 94 & 391&1998 \\
    Interaction and outeraction: instant messaging in action & 90 & 1225&2000 \\
    Providing presence cues to telephone users & 83 &177 &2000 \\
    Design of a multi-media vehicle for social browsing & 72 &331 &1988 \\
    Distributed multiparty desktop conferencing system: MERMAID & 69 &153 &1990 \\
\midrule
\multicolumn{4}{c}{\textbf{UIST}} \\
\midrule
    Sensing techniques for mobile interaction & 254 & 592&2000 \\
    The world through the computer: computer augmented interaction with real-world environments & 227 & 487&1995 \\
    HoloWall: designing a finger, hand, body, and object sensitive wall & 197 & 243&1997 \\
    A survey of design issues in spatial input & 166 & 417&1994 \\
    Tilting operations for small screen interfaces & 158 &412 &1996 \\
    Multi-finger and whole hand gestural interaction techniques for multi-user tabletop displays & 156 &527 &2003 \\
    DiamondTouch: a multi-user touch technology &153 & 1336&2001 \\
    The document lens & 135 & 416&1993 \\
    The DigitalDesk calculator: tangible manipulation on a desk top display & 132 & 324&1991 \\
    Pad++: a zooming graphical interface for exploring alternate interface physics & 131 &754 &1994 \\
\midrule
\multicolumn{4}{c}{\textbf{UbiComp}} \\
\midrule
    Validated caloric expenditure estimation using a single body-worn sensor & 113 & 83&2009 \\
    InfoScope: Link from Real World to Digital Information Space & 67 &34 &2001 \\
    Self-Mapping in 802.11 Location Systems & 63 &130 &2005 \\
    The NearMe Wireless Proximity Server & 62 & 162&2004 \\
    Predestination: Inferring Destinations from Partial Trajectories & 51 &498 &2006 \\
    UbiTable: Impromptu Face-to-Face Collaboration on Horizontal Interactive Surfaces & 40 &261 &2003 \\
    Accurate GSM Indoor Localization & 37 & 537&2005 \\
    Very Low-Cost Sensing and Communication Using Bidirectional LEDs & 34 & 157&2003 \\
    Particle Filters for Location Estimation in Ubiquitous Computing: A Case Study & 33 & 254&2004 \\
    PowerLine Positioning: A Practical Sub-Room-Level Indoor Location System for Domestic Use & 31 &152 &2006 \\

    \bottomrule
\end{tabular}
}
    \caption{Top CHI, CSCW, UIST and UbiComp papers cited by patents. The majority of them are highly-cited papers in academia whose major contribution is a system.
    }
    \label{tab:top_HCI}
\end{table*}


\subsection{RQ2: Who is patenting and who is producing patent-cited papers?}
We next investigated the top patent assignees that cite HCI papers.

\textbf{Top patent assignees that cite HCI research over time.} We examined who are the top patent assignees (the entity that has the property right to the patent, e.g. firm) that cite HCI research. The top patent assignees have been dominated by companies (Figure~\ref{fig:f7}): Apple, Microsoft, and International Business Machines Corporation (IBM) are the top three companies that were granted the highest number of HCI-citing patents in the dataset. Other rise and fall over time: for example, from $1990$ - $2005$, top patent assignees were companies such as Xerox Corporation, Fuji, and Siemens; since 2010, the top patent assignees were Apple, Google, and Amazon. % indicating industry companies do value HCI research to a great extent. %{DM: just shows top companies patent things more, no?}

\hancheng{not sure where this paragraph goes}
\msb{Unless this is specifically about institutions that write PATENT-CITED papers, I don't understand what this is doing in the paper}
\textbf{Top institutes that publish HCI papers over time.} At the same time, we assessed the institutes that published the highest number of HCI papers across years. As Figure ~\ref{fig:f11} shows, contrary to the fact that top patent assignees are dominated by industries, top HCI paper institutes are mainly universities, i.e. Carnegie Mellon University, Massachusetts Institute of Technology,  University of Washington, etc. There were also companies that published a large number of HCI papers such as Xerox Palo Alto Research (before 2005) and Microsoft (after $2005$). Moreover, we also observed a decreasing fraction of HCI papers being cited by patents from $1990$ to $2020$.% {DM: Again, kinda obvious. These are top universities for HCI research, no?}

\textbf{Self-citation.} We also explored the degree of self-citation, which refers to the authors of research papers turning the research into patents. Although the number of self-citing patents is growing, the percentage of self-citations in all HCI patent citations is decreasing. This suggests that while the HCI field is expanding, the number of researchers directly referring their own research in patents is not growing at the same rate. \msb{I'm not really sure what's to be taken away from this analysis. Cut?}% which will be discussed more with details in Section \ref{sec:patent_recognize}. {DM: this may be because patenting and research are growing more specialized, so you are less likely to do both, whereas in past when HCI was young, you could.}



\begin{figure}[t]
    \centering
    \includegraphics[width=1.\linewidth]{main_figs/fig3.pdf}
        \caption{Top patent assignees that cite HCI research over time. \msb{The text in this graph is too small to read. I suggest picking fewer institutions per graph (say, top 5-7), and making the font size much larger. Please also decapitalize TITLES THAT ARE ALL CAPS and Title case the graph title. You don't need to repeat the same graph title over every facet of the graph.}} 
    \label{fig:f7}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=1.1\linewidth]{main_figs/fig4.pdf}
        \caption{Institutes that publish most HCI papers over time, and the proportion of their published papers that are recognized by patents. \msb{Same critique as the prior figure. Also, I suggest removing 2015-2018}} 
    \label{fig:f11}
\end{figure}

%\paragraph{\textbf{Who is patenting:Top patent assignees that cite HCI research over time}
% patent terms; modalities; system interaction; evaluations; theory; social and experience design; input techniques
% paired t-test
% regression percentage ~ year


\subsection{RQ3: Paper Content vs. Patent Content} \label{Paper Content vs. Patent content over time}
%\yt{Maybe Yujie add more details of LDA here?} Finally, we dissected the content of the papers and patents and analyzed their content evolution over time. 
Which HCI research topics are the focus of industry activity? To answer this question, we compare published HCI research to patent-cited HCI research via Latent Dirichlet Allocation (LDA), a classic method of topic modelling \cite{blei2003latent}. LDA  automatically discovers topics within documents, where each topic is represented as a probability distribution of words. Each document can also be represented as a probability distribution over different topics. 

We concatenated each paper title with its abstract to represent its contents. Similarly, we concatenated each patent title with its abstract to represent the patent's contents. We then tokenized the text corpora into unigrams and bigrams, filtered out terms that appear fewer than 5 times in the corpus, removed stop words in English, and then ran LDA modeling. We varied the number of topic and aligned on seven topics as resulting in the highest quality topics. \msb{Do not use Topic 1, Topic 2,  or numbers like that in the figure --- they are impossible to remember. Give each topic a representative title instead.} Figure~\ref{fig:topic_fig2} reports the result. It can be inferred that topic $0$ is related to patents, topic $1$ to multi-modality, topic $2$ to UI systems, topic $3$ to sensing methods, topic $4$ to design, topic $5$ to social computing, and topic $6$ to input techniques. 

We then compute the topic distributions for each document (paper or patent) in our corpus, then aggregate topic distributions of all documents within a specific year that belong to certain document category (patents, patent cited papers, or non-patent cited papers) so as to get an estimated number of documents that belong to a particular topic for that document category for a particular year. In the first row of Figure~\ref{fig:topic_fig3}, we plotted the topic distribution for patent-cited HCI papers (left), non-patent cited HCI papers (middle) and patents (right), i.e., how many papers belong to topic X in year Y. %We can observe two patterns by comparing the three diagrams. 
%First, it can be observed that the absolute total number of papers for patant-cited HCI papers, non-patent cited HCI papers, and patents have similar overall distributions: all peaked at certain years ($2010$ - $2015$) and then quickly went down, which is consistent with the trend of total patent citation in Figure 1\ref{fig:f1}, though the peaks did not occur in the same year (the patent cited at $2012$, the patent cited at $2017$ and patent at $2014$). Moreover, 
%We could see that the topic distribution is uneven for each category and each category's topic distribution are quite different and varies by their own over time.
%\hancheng{mention the exact topic}
%\hancheng{to add explanation}
The second row of Figure~\ref{fig:topic_fig3} normalizes this topic distribution, i.e., what is the proportion of topic X in year Y for a specific document category, to better illustrates the distribution pattern. 


\msb{I struggle to make much sense of this section. It's just a list of stuff that happened, but I don't know how to connect it to a narrative. What if you invert the organization and instead take it topic by topic? Sort by decreasing popularity, so start with the most popular one, define it, explain how popular it is (e.g., 50\% of all patent cited papers overall) and then describe any temporal trends (e.g., getting smaller over time)}

Topic $2$ (systems) has dominated the patent-cited HCI papers over time, indicating system oriented research has been of considerable importance in patent-cited HCI research. In patent-cited papers, initially from $1980$ to $1990$, the distribution is dominated by topic $1$ (multi modality), topic $2$ (system) and topic $4$ (design theory) while the proportion of topic 5 and 6 remained low. Since 1990, the proportion of topic $5$ and $6$ gradually increases while topic $2$ (system), topic $3$ (sensing method) and topic $4$ (design theory) shrank. Then, topic $2$ (system) began expanding again and topic $3$ (sensing method) and topic $5$ (social computing) shrinks again while topic 6 (input technologies) kept increasing. 

The topic distribution of non-patent cited papers shows a similar trend yet the expansion of topic $5$ (social computing) since $1990$ is more rapid and that of topic 6 is less rapid compared with that in patent-cited case. Additionally, the re-expansion of topic $2$ (system) since $2014$ is less significant than that in the patent-cited case. Taking a look at recent years, we observed that the non-patent cited papers are mainly dominated by topic $4$ (design theory), and topic $5$ (social computing), which are behaviour analysis such as design theory and social computing, from $2015$ to $2020$. 

On the contrary, the topic distribution of patents shows a very different trend. Since 1990, the topics have been dominated by topic 0 and topic 6. While the proportion of topics 1-5 remains the same, topic $0$ (patent) first shrinks from 1990 to 1993, then gradually expands form 1993 to 2010 and shrinks again since $2010$ \msb{does this really mean anything? what does it mean for this topic to grow?}. This trend of topic $0$ (patent) is in contrast to that of topic 6, which first expands from $1990$ to $1993$, then slightly shrinks from $1993$ to $2010$ and expands again since $2010$. Nearly half of patents belong to topic \msb{???} from $1990$ - $2015$, which makes sense since topic $0$ (patent) is about patent. 


It is worth noticing that proportion of topic $6$ (input techniques) in both the patent-cited HCI papers and patents have increased significantly since $2010$, which indicates that there is growing number of patent-cited HCI papers and patents on input techniques.%\yt{Maybe this is something interesting but not sure how to interpret it} 

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{analysis_figures/topic_fig1.png}
%     \caption{\hancheng{not necessary we are good with topic=7}} 
%     \label{fig:topic_fig1}
% \end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{analysis_figures/topic_fig2.png}
    \caption{Combining papers and patents as one corpora with LDA and topic number of $7$. Topic 0 relates to patent terms, topic 1 is on modalities, topic 2 is likely on system interaction, topic 3 is on evaluations, topic 4 is on theory, topic 5 is on social and experience design, topic 6 is on input techniques \msb{see earlier comment about topic numbers being not useful}} 
    \label{fig:topic_fig2}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{main_figs/topic.pdf}
    \caption{The first row shows the breakdowns of papers across $7$ topics in HCI over time. The second row depict the percentage of each topic in terms of paper number. Three columns depict "topic distribution of patent-cited HCI papers", "topic distribution of non-patent cited HCI papers" and "topic distribution of patents" respectively. From the second row, we can observe that for patent-cited papers, Topic 1, 2, has been dominating from 1980 to 1990. Topic 5 and 6 expands while topic 2, 3 and 4 shrinks since 1990. Topic 2 starts expanding while topic 3 and 5 shrinks again till 2014. For non-patent-cited ones, we observe a similar trend. For the patents, Topic 0 and Topic 6 have been dominating since 1990. Topic 0 first shrinks from 1990 to 1993, expands from 1993 to 2010 and shrinks again since 2010, in contrary to the trend of Topic 6. \msb{see my comment overall on the section. this caption is too much high resolution information, and a reader's brain will just skim it rather than take one or two big ideas away. What should they be learning from these figures?} \msb{Figure legend isn't useful, axis titles aren't right (not capitalized, it says percentage but outcome isn't a \%)}} 
    \label{fig:topic_fig3}
\end{figure}

%\paragraph{\textbf{venue comparison}}
%?
\subsection{RQ4: What types of HCI papers are more likely to be in patents?}
\msb{This subsection feels like it has no consistent theme, and should be blown apart and the results inserted into the appropriate sections}

To understand what types of HCI papers are more likely to be transferred into patents, we analyzed both the patent-recognized and non patent-recognized HCI papers from $1980$ to $2018$ through comparing their academic impact, content, and origins. 

\paragraph{\textbf{High impact papers in academia are more likely to be recognized by patents}}
We further investigate how academic impact relates to patent impacts, measured by the paper's number of citations from other academic papers (academic citation count) and number of citations from patents (patent citations count). % we assessed the relationship between paper's aggregated number of citations by other papers and the paper's aggregated number of citations by patents. 
Figure~\ref{fig:f3}a) shows the academic citation count for both papers recognized by patents and papers not recognized by patents. Papers recognized by patents generally have more academic citations than those not recognized by patents. \msb{to conclude this, you'd want to do an unpaired t-test between the two conditions. but see comment below: these are not normally distributed quantities, so you'd either need to log transform or use a nonparametric equivalent such as a Mann-Whitney U}

\msb{A couple issues with this analysis. One is presentation: since there are only four correlation coefficients, I suggest reporting them directly in the text rather than in a table figure. The second is analysis: citation and patent citations are exponentially distributed most likely, which makes a correlation coefficient a poor model since it assumes a normally distribution. Either take a log of both quantitites before computing the correlation, or use a nonparametric equivalent such as a rank correlation instead.} We also studied the Pearson correlation between paper's academic citation count and the paper's patent citation count. The positive correlation and the significant p-value in Figure~\ref{fig:f3} b) further validates that highly-cited papers in academia are more likely to be recognized by patents in a significant way. Comparing across different venues, we observed greatest correlation for UIST, followed by CSCW, CHI and UbiComp. %This concludes that papers with more academic citations are more likely to be recognized by patents.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{main_figs/fig7abc.pdf}
    \caption{Top left: papers cited by patents receive more academic citations in HCI. \msb{I suggest cutting parts b and c, as well as the rest of this text} We also visualize paper-wise by venue, with x axis as paper citations and y axis as patent citations, and study their Pearson Correlation. The positive correlation suggests highly-cited papers in academia are more likely to be cited by patents.} 
    \label{fig:f3}
\end{figure}


\paragraph{\textbf{Applied papers more likely to be recognized by patents}}
%\yt{but we also have bigrams?}
\msb{This all feels like it should go with the topic discussion}
We further examined whether papers' content influences its recognition by patents. Using the topics that were clustered by LDA in Figure\ref{fig:topic_fig2}, we observed that patent-recognized patents are mostly from Topic $0$ (patent), Topic $2$ (system), and Topic $6$ (input techniques), which relate to patent, system, and input techniques correspondingly. On the opposite, non-patent recognized papers are mostly from Topic $4$ (design theory) and Topic $5$ (social computing), which relate to design theory and social computing. \msb{Can you make those claims without a statistical test?} These patterns are largely consistent with the earlier quantitative analysis in Section \ref{Paper Content vs. Patent content over time}: the topic distribution of patent cited paper are largely dominated by applied techniques (Topic $0$ and Topic $6$), but the topic distribution of non-patent cited paper are largely dominated by behaviour studies such as Topic $4$ (design theory) and Topic $5$ (social computing). \msb{again, if you want to claim something is ``more'' or ``less'' than another category, you need a statistical hypothesis test} 

\msb{It's not clear that a TF-IDF analysis adds anything material to the analysis beyond the topic analysis. I would do one or the other, but not both}
Moreover, we conducted analysis at term level through comparing terms of patent-cited and non-patent cited papers. We first lemmatized the text, then leveraged TF-IDF to weight the importance of unigrams and bigrams that appear in at least 1\% of documents but no more than 80\% documents, and studied their distribution. Figure~\ref{fig:f4} lists the top $25$ terms ranked by TF-IDF score for both papers recognized by patents and those not recognized. 
%Although some unigrams are present in both categories, such as "user", "use" and "interface", the rankings are different in the two categories for these shared ones. Moreover, 
%Although some terms are present in both categories, some top ranked terms that occur in the papers recognized by patents, such as "applications",  are not present in papers not recognized by patents. These missing unigrams suggest that papers related to applied purposes are more likely to be recognized by patents. With a logistic regression model using TF-IDF features, we are able to classify whether a paper gets cited by patents or not with AUC 0.76, indicating significant difference in language usage for papers cited by patents and those didn't.
Although some terms are present in both categories, some top ranked terms that occur in the papers recognized by patents, such as "interface", "display", "touch" and "technique",  are not present in papers not recognized by patents. These missing unigrams suggest that papers related to applied purposes are more likely to be recognized by patents. With a logistic regression model using TF-IDF features, we are able to classify whether a paper gets cited by patents or not with AUC 0.76, indicating significant difference in language usage for papers cited by patents and those didn't. The significant coefficients of logistic regression are presented in Fig.\ref{fig:f5}. As can be seen, terms related to application and system building such as `technique', 'implement', 'interface', 'evaluation' are associated with patent citation while terms more associated with behavioral works or theories such as `understand', `reflect', `opportunity', `future' and associated with no patent citation.


%\hancheng{use some results from LDA in section 1, e.g. describe difference between topics that differ in amount} \yt{Done.}

\begin{figure}[t]
    \centering
    \includegraphics[width=.7\linewidth]{main_figs/fig4.pdf}
        \caption{Top terms weighted by TF-IDF in non-patent cited papers and patent cited papers.} 
    \label{fig:f4}
\end{figure}

\begin{figure}[t]
    \centering
    \includegraphics[width=.8\linewidth]{main_figs/fig5.png}
        \caption{Top terms that predict patent citation.} 
    \label{fig:f5}
\end{figure}

\paragraph{\textbf{Industry papers have higher percentage of papers cited by patents than academia for top institutes}}
\msb{this feels like it's about the `who', and should move}
We analyzed the institute affiliations of patent-cited and non patent-cited HCI papers for top institutes that publish the most HCI papers. Figure~\ref{fig:f6} shows the number of papers recognized and not recognized by patents for different institutes. We find $35.5\%$ of Microsoft’s papers , $31.0\%$ of IBM’s and $65.1\%$ of Xerox’s were recognized. In comparison, university has a lower rate of papers cited by patents, e.g. 25.2\%, 15.3\%, 26.9\% of papers were recognized among Carnegie Mellon University, University of California systems and MIT respectively. This indicates that among institutes publishing the most HCI papers, the papers from industry have a higher proportion of papers recognized by patents. \msb{Is this still true if you remove the self-citations?} %\yt{Maybe it's better to label the percentage of papers recognized on Figure~\ref{fig:f6}} 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\linewidth]{main_figs/fig6.png}
        \caption{Industry papers have higher percentage of papers cited by patents for institutes that publish most HCI papers.} 
    \label{fig:f6}
\end{figure}

\paragraph{\textbf{Self-driven technology transfer}} \msb{this figure is nowhere near the text it references} Figure \ref{fig:f8}a) shows the number of self-citing patents over years and clearly this number has increased rapidly since 1995. Figure \ref{fig:f8}b shows the percentage of self-citing patents in all patents over years and we can observe that the percentage took off in $1991$ and peaked in 2000 and gradually decreased since $2000$. This suggests that although the overall self-citing patent number has increased, the proportion of self-citing patents does not follow a monotonic trend.


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{main_figs/selfcite.pdf}
        \caption{Self-cite: patent inventors refer to their own research papers in patents.} 
    \label{fig:f8}
\end{figure}

\subsection{RQ5: How long does it take for patents to recognize papers}
\label{sec:patent_recognize}
How long does it take for patents to recognize papers? To examine this question, we investigated the time lag between patent and paper. 

%\hancheng{add some results on aggregated time lag}
\paragraph{\textbf{Time lag between patent and paper is long, and getting longer.}}
To measure how long does it take for HCI paper to be recognized patents, for each patent, we measured the time lag between the issue date of the patent and the publication date of all HCI papers it cited. We measure the lag from patent backward, rather than from paper forward, because we cannot know whether a paper will receive a citation but has not yet, but we can know how far back a patent's citations reach.

In our dataset, the average patent-paper lag is 10.45 years \msb{report stdev}, indicating that patents on average reference HCI research papers published 10.45 years before the patent filing date. 


We then studied how the time lag varies over time by grouping the patent-paper time lag at patent level while aggregating in different ways, e.g. the average.median \msb{?} time lag between patent date and the publication date of all HCI papers the patent cite, or the time lag between patent date and the publication date of the most recent HCI paper it cited. \msb{For both the paper and the figure, take a position on what the correct statistic should be. Right now this section and figure are buried in a lot of high resolution information going between different measures. I would focus the figure on just one, and the text as well. You can bring up the other statistics if they have specific interesting results, rather than covering them all. My vote would be median.}
As Figure~\ref{fig:f9} a), c) shows, the average difference between the time the cited paper is published  and the time the paper is cited by the patent, is becoming larger from 1989 to 2014 for all the venues. However, since $2014$, this trend bifurcates among different venues: the time lag for CSCW increases to over 20 years and Ubicomp decreases to about 10 years at 2017. \msb{in both figure and text, it should be Ubicomp and not UBI} In the mean time, we also examined the time lag between the patent and its most recent paper, which is shown in Figure \ref{fig:f9} b). It can be observed that for a patent, the difference between the time its most recent paper was published and the time it is patented also becomes larger from $1989$ to $2011$ for all the venues. \msb{throughout this section, trends are reported without numbers. What does longer mean? How much longer? Is this difference significant?} This increase gradually slowed down, leading to a slight decrease since $2011$ for all the venues. At $2018$, the time lag for CSCW and CHI still remained over $10$ years while UIST and UBI's went below $10$ years. We observed similar patterns when aggregating the time lag when considering the median time lag between patent date and the publication date of papers they referred to. Across venues, we find that CSCW generally takes the longest time to be recognized by patents, while UIST and UbiComp takes shorter time, which could be explained by the fact that more system-driven works are likely to diffuse more quickly into pracice. \msb{When I look at medians, the conferences look pretty indistinguishable to me, except maybe Ubicomp (blue)}

\msb{if you focus on median in the prior paragraph, then you can have a brief paragraph here that reports general trends on the most recent paper, which looks like it's stretched from around five years in 1995 to ten years in 2005 to 11 or 12 years in 2015}

The patent citation also involve different sources, some are added by the applicants/inventors, while others are added by patent examiners. The dataset we used also provide a breakdown of reference types, including applicant/inventor added (app), examiner added (exm), other (oth), and unknown (unk) types. As shown in Figure \ref{fig:f9} d), references added by patent examiners are generally more recent than what inventor added, although similar trend of long time lags and increasing time lags still are still observed. \msb{not sure you need a figure for this}

All results here indicate that patents mostly cite old research, and is citing increasingly older research, which holds true across venues, and reference types, indicating HCI research generally does not have immediate impacts on patent. \msb{Again, we need to separate out that I'm citing a canon of prior work that's getting older at a rate of one year per year, from I'm citing recent work but the recent work I'm citing is not as recent as it used to be} This conclusion is largely identical to what is found in science in general \cite{marx2022reliance}.
%\yt{Not sure how to interrupt Figure~\ref{fig:f9} c). Needs more discussion. Also it could be easier to describe if we define patent-paper time lag in the methods, as in Figure~\ref{fig:f10}} 
% \yt{Maybe 2018, double check the year on the graph}
%\hancheng{describe how the time lag is calculated, also add a sentence or two how different venues differ} \yt{done. Fig 11 (c) needs to be added. @hancheng } 
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{main_figs/fig12.pdf}
        \caption{Time lag between patent and paper is long and getting longer for different types of citations and venues}.%\hancheng{one time lag of the most recent paper should be substituted with median time lag}} 
    \label{fig:f9}
\end{figure}


\paragraph{\textbf{Self-driven translation tends to be faster}}
The other interesting feature of patent translation's time pattern is that 
those self-cite patents have a shorter patent-paper time lag compared with those non-self-cite. As Figure~\ref{fig:f10} shows, from $1990$ to $2008$, the patent-paper time lag for self-cite patents remains slightly lower than the non-self-cite  in most of the years. Since $2008$, the time lag for the non-self-cite one increased rapidly and was beyond 175 months in $2018$ while the self-cites remain below $75$ months. This suggests that papers transferred faster by authors themselves into patents, compared with those transferred by others, and this speeding up has become more significant since $2008$. \msb{I think this can likely all be compressed down to 1-2 sentences, and no figure needed}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.5\linewidth]{main_figs/fig10.png}
        \caption{Self-driven translation tends to be faster} 
    \label{fig:f10}
\end{figure}

%\paragraph{\textbf{venue comparison}}
%\hancheng{UIST is getting shorter! discuss this}
%\hancheng{why the data ends at 2018}

\textbf{Summary of conclusions:} Through our analysis, we find that HCI research has had significant impact on patents, with increasing number of patents recognizing research in CHI, CSCW, UIST and UbiComp; Patents are more likely to refer to systems-oriented and highly-cited research in academia. However, the time lag between patent and paper is long (>10 years) and getting longer, suggesting HCI research and practice may be inefficiently connected. 

\msb{I don't think this should go after your summary}
\textbf{Robustness check:} Apart from conducting analysis on full citation data, we also run two additional analysis as robustness checks to further verify our findings, which we include in the Appendix. To rule out the possibility that the impacts of HCI research on patents is a result of self-citations, or driven primarily by HCI researchers --- thus one may argue the impact of HCI research in industry is actually limited --- we run the same analysis using patents that 1) do not include self-citations to one's own research papers (Appendix A.1), and 2) patents that are invented by people who have never published any HCI research papers (Appendix A.2.), by selecting the set of inventors whose last name never appears in any of the author lists of our studied HCI research papers. This results in $5251$ ($17.12\%$) of patents that involve no researcher last time \msb{I don't understand that phrase} and $26382$ ($86.04\%$) patent involve non self-cite citations. We find consistent patterns as our main analysis where a high proportion of HCI research papers are cited by those patents. Similarly, the patterns of time lag hold for additional analysis.
